Antipodes of Label Differential Privacy: PATE and ALIBI

We consider the privacy-preserving machine learning (ML) setting where the trained model must satisfy differential privacy (DP) with respect to the labels of the training examples. We propose two novel approaches based on, respectively, the Laplace mechanism and the PATE framework, and demonstrate their effectiveness on standard benchmarks. While recent work by Ghazi et al. proposed Label DP schemes based on a randomized response mechanism, we argue that additive Laplace noise coupled with Bayesian inference (ALIBI) is a better fit for typical ML tasks. Moreover, we show how to achieve very strong privacy levels in some regimes, with our adaptation of the PATE framework that builds on recent advances in semi-supervised learning. We complement theoretical analysis of our algorithms' privacy guarantees with empirical evaluation of their memorization properties. Our evaluation suggests that comparing different algorithms according to their provable DP guarantees can be misleading and favor a less private algorithm with a tighter analysis. Code for implementation of algorithms and memorization attacks is available from https://github.com/facebookresearch/label_dp_antipodes.

==> checklist.tex <==
\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} \textit{See Section~\ref{apx:attack} in Supplemental results.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} \textit{The code is included in the supplemental materials.}
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} \textit{See Section~\ref{s:evaluation}.}
    
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} \textit{All reported accuracies are stable $\pm .5\%$, empirical privacy estimates (Table~\ref{table:comparitive-results}) are reported as 95\%-confidence intervals.}
    
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} \textit{We cite Kim~\cite{fixmatchpytorch}, Krizhevsky~\cite{Krizhevsky09learningmultiple}, Papernot et al.~\cite{papernot2018scalable}, Liu~\cite{resnet-source}, and Zagoruyko and Komodakis~\cite{WideResNet}.} 
  \item Did you mention the license of the assets?
    \answerYes{} \textit{We list licenses for code where available.}
    
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} \textit{The supplemental materials include training code and implementation of memorization attacks.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> dpl-sgd.tex <==
We will be using the following notation. Inputs into the model are pairs of \((x_i, y_i)\), where \(x_i\) is a feature vector and \(y_i\) is the label. The model \(M\) is parameterized with a vector of weights, \(W=(w_1,...,w_d)\). For simplicity, assume that we are training a binary classifier, whose output is the probability (or, more generally, a scalar real number), and the loss function \(\matchscr{l}(M(W, x_i), y_i)\) is cross-entropy. Training is performed with mini-batches of size B.


As we know, this algorithm preserves privacy of the (xi, yi) pairs, and it is the most natural way of doing it. Why is that? Because each g̃i  is dependent on the secret inputs, and the additive Gaussian mechanism is the basic mechanism for releasing multi-dimensional sums of vectors with bounded L2 norm.

However, the cost of this mechanism is rather high, because it clips the L2 norm of the d-dimensional per-sample gradient gi, but it adds noise as if the entire vector had support on a single coordinate and that coordinate could be anywhere.

more an more ...

The new algorithm, let’s call it DPL-SGD (DP for Labels SGD)


\begin{algorithm}[H]
\SetAlgoLined
\For{ $(x_i, y_i) \in $ mini-batch}{
    compute (zi, gi') from ∇ Loss(M(W, xi), yi) where gi' = gi  / zi 
	compute ub = maxi |gi'|  - d-dimensional coordinate-wise max of absolute values
    compute G = (�� gi + Nd(0, d · (ub · ��)2)) / B  - the normal noise has variance d · (ubi · ��)2 in the i’th coordinate
    update W with G
}
\caption{DP-SGD}
\end{algorithm}

Note that DPL-SGD does not clip gradients, which is already a win over DP-SGD.

==> rr_eps.tex <==
\section{Soft Randomized Response with Post-Processing: Privacy Analysis}\label{a:rr_eps}
Privacy budget analysis of the additive noise Soft-RR is similar to the analysis in Dwork et al.~\cite{dwork2014algorithmic} with the exception that the sensitivity of the function, i.e. the soft label [or one-hot label in our setting], is equal to $\sqrt 2$ regardless of the number of classes. This is because $D$ and $D'$ do not differ in a single element in our local privacy setting. The attacker is instead trying to distinguish between two PMFs ($p$ and $q$) whose difference is upper bounded by $\lVert p(.) - q(.) \rVert = \sqrt 2$.

We also derive a generic formula to calculate the privacy budget given the assumption that the added noise is applied independently on elements of label presented as a one-hot vector. Assuming $C$ is the set of classes we show a one-hot label by $y_c = \{[c = k] | k \in C\}$, where $[\cdot]$ is Iverson bracket.

We further assume -- without loss of generality -- that the added noise noise has mean $0$ and standard deviation $\sigma$, we show this as $\eta_{0, \sigma}$.
Let's Assume $y_c$ and $y_d$ are two labels that we would like to distinguish given the mechanism output $\mathbf{o}$. We would like to calculate the bound on:

\begin{equation}
    R_{c, d} = \frac{P(\mathbf{o} \big| y_c)}{P(\mathbf{o} \big| y_d)}
    \quad \forall c, d \in C
 \end{equation}
Given $\mathbf{o} = {(o_0, o_1, \ldots o_{C-1})}$ and the fact that
$o_l$ are i.i.d, only the two terms with corresponding to indices $c$ and $d$ remain.
\begin{equation}
    \label{simple_ratio}
    R_{c,d} = \frac{p(o_c\small|\eta_{1, \sigma})p(o_d\small|\eta_{0, \sigma})}{p(o_c\small|\eta_{0, \sigma})p(o_d\small|\eta_{1, \sigma})}
\end{equation}
\subsection{Laplace Mechanism and $\eps$-privacy}
With a Laplace mechanism we would like to find an $\eps$ such that:
\begin{equation}
    \label{laplace_rr_bound}
    \max(R_{i,j}) < e^{\eps}
\end{equation}
Given a Laplace with standard deviation $\sigma$ we will have:
\begin{align*}
    \max(R_{i,j}) &= \max(\frac{e^{-\sqrt 2 \small|o_i-1\small|/\sigma}e^{-\sqrt 2 \small|o_j\small|/\sigma}}{e^{-\sqrt 2 \small|o_i\small|/\sigma}e^{-\sqrt 2 \small|o_j-1\small|/\sigma}}) \\
    &= \max(e^{{-\sqrt2}\frac{(\small|o_i\small| - \small|o_i-1\small|) - (\small|o_j\small| - \small|o_j-1\small|)}{\sigma}})\\
    & \leq e^{2 \sqrt 2 / \sigma}
\end{align*}
Thus we will have:
\begin{equation}
    \label{laplace-eps}
    \eps = \frac{2\sqrt2}{\sigma}
\end{equation}
\subsection{Gaussian Mechanism and $(\eps, \delta)$-privacy}
For Gaussian noise we can have a $(\eps, \delta)$-privacy such that:
\begin{equation}
    \label{gaussian_rr_bound}
    \Pr(\max(R_{i,j}) \geq e^{\eps}) \leq \delta
\end{equation}

the eq. \ref{simple_ratio} becomes:
\begin{align*}
    \max(R_{i, j}) &= \max(\frac{e^{-(o_i - 1)^2/2\sigma^2}e^{-(o_j)^2/2\sigma^2}}{e^{-(o_j - 1)^2/2\sigma^2}e^{-(o_i)^2/2\sigma^2}}) \\
    &= e^{\small|o_i + o_j\small|/\sigma^2}
\end{align*}
Following the same logic as in Dwork et al.~\cite{dwork2014algorithmic}. Eg. \ref{gaussian_rr_bound} is bounded by $\eps$ if $\small|o_i + o_j\small| < \sigma^2 \eps$. 
We can replace $x=o_i + o_j$ with a single R.V. sample $x$ from $\eta_{0, \sqrt{2}\sigma}$, thus we will need:
\begin{equation}
    \label{gaussian_rr_delta}
    \Pr[\small|x\small| \geq \sigma^2 \eps] < \delta  \quad \Leftrightarrow \quad \Pr[x \geq \sigma^2 \eps] < \delta / 2
\end{equation}
In ~\cite{dwork2014algorithmic} the following tail bound is used to drive a formula for $(\eps, \delta)$ based on $\sigma$ :
\begin{equation*}
    \Pr[x > t \small| x \sim \eta_{0, \sqrt{2}\sigma}] \leq \frac{\sigma}{t\sqrt{\pi}} e^{-t^2/4 \sigma^2}
\end{equation*}
This bound is loose and for practical purposes Eq. \ref{gaussian_rr_delta} is enough to get a tighter bound on these values using look-up tables.

